Revisiting Explicit Negation in Answer Set Programming

A common feature in Answer Set Programming is the use of a second negation, stronger than default negation and sometimes called explicit, strong or classical negation. This explicit negation is normally used in front of atoms, rather than allowing its use as a regular operator. In this paper we consider the arbitrary combination of explicit negation with nested expressions, as those defined by Lifschitz, Tang and Turner. We extend the concept of reduct for this new syntax and then prove that it can be captured by an extension of Equilibrium Logic with this second negation. We study some properties of this variant and compare to the already known combination of Equilibrium Logic with Nelson's strong negation. Under consideration for acceptance in TPLP.

==> abbreviations.tex <==
%!TEX root = main.tex

\makeatletter
\def\renewtheorem#1{%
  \expandafter\let\csname#1\endcsname\relax
  \expandafter\let\csname c@#1\endcsname\relax
  \gdef\renewtheorem@envname{#1}
  \renewtheorem@secpar
}
\def\renewtheorem@secpar{\@ifnextchar[{\renewtheorem@numberedlike}{\renewtheorem@nonumberedlike}}
\def\renewtheorem@numberedlike[#1]#2{\newtheorem{\renewtheorem@envname}[#1]{#2}}
\def\renewtheorem@nonumberedlike#1{  
\def\renewtheorem@caption{#1}
\edef\renewtheorem@nowithin{\noexpand\newtheorem{\renewtheorem@envname}{\renewtheorem@caption}}
\renewtheorem@thirdpar
}
\def\renewtheorem@thirdpar{\@ifnextchar[{\renewtheorem@within}{\renewtheorem@nowithin}}
\def\renewtheorem@within[#1]{\renewtheorem@nowithin[#1]}
\makeatother

% \definecolor{lightgray}{gray}{0.9}
% \newcommand{\highlight}[1]{\colorbox{lightgray}{$\displaystyle #1$}}


% \newcommand{\reg}[1]{\mathit{reg(#1)}}
% \newcommand{\ctxtfree}{\mathit{ctxtfree}}
% \newcommand{\nComp}{\mathit{nComp}}
% \newcommand{\ASP}{\mathit{ASP}}
% \newcommand{\CalPI}{\CalP I}
% \newcommand{\tranN}{\mathit{tranN}}

\newcommand{\modif}{\mathsf{mod}}

% \newcommand{\Pdisj}{\CalP^{\vee}}

\newcommand{\Pex}{\CalP_{\mathsf{1}}}

\newcommand{\Pexx}{\CalP_{\mathsf{2}}}





\newcommand{\CalI}{{\cal I}}
\newcommand{\CalL}{{\cal L}}
\newcommand{\CalS}{{\cal S}}
\newcommand{\CalP}{{\cal P}}
\newcommand{\CalQ}{{\cal Q}}
\newcommand{\CalM}{{\cal M}}
\newcommand{\CalA}{{\cal A}}

\newcommand{\Psneg}{\tilde{\CalP}}

\newcommand{\udf}{\mathsf{U}}
\newcommand{\true}{\mathbf{\top}}
\newcommand{\false}{\mathsf{\bot}}

\newcommand{\True}{\textit{true}\xspace}
\newcommand{\False}{\textit{false}\xspace}

\newcommand{\Ground}{\mathsf{g}}
\newcommand{\atoms}{\mathsf{at}}
\newcommand{\Atoms}{\mathsf{At}}
\newcommand{\ATOMS}{\CalA\mathsf{t}}
\newcommand{\AUXATOMS}{\mathsf{auxatoms}}
\newcommand{\nA}{n\_A}
\newcommand{\Head}{\mbox{\em Head}}
\newcommand{\Body}{\mbox{\em Body}}
\newcommand{\ud}{\mathsf{undef}}
\newcommand{\Def}{\mathsf{def}}
\newcommand{\defname}[1]{\textit{#1}}

\newcommand{\as}{\mathsf{as}}
% \newcommand{\asp}{\mathsf{as}}
\newcommand{\wc}{\mathsf{wc}}
\newcommand{\As}{\mathsf{As}}
\newcommand{\NAs}{\mathsf{NAs}}

% \newcommand{\ctxt}{\mathsf{\neg}}
\newcommand{\ctxt}{\mathsf{ctxt}}
\newcommand{\naf}{\mathsf{naf}\,}
\newcommand{\nlnot}{\mathsf{not}\,}
\newcommand{\Fp}{\mathsf{fp}\;}
\newcommand{\Lfp}{\mathsf{fp}\,}
\newcommand{\Svl}{\Phi}
\newcommand{\Pctxt}{\CalP_{\ctxt}}

\newcommand{\Svlp}{\Phi_{\CalP}}
\newcommand{\ModelsWCS}{\models_{wcs}}

\newcommand{\Luka}{\L}

\newcommand{\Penguin}{\mathit{penguin}}

\newcommand{\fly}{\mathit{fly}}
\newcommand{\Fly}{\mathit{can\_fly}}
\newcommand{\Ab}{\mathit{ab}}
\newcommand{\Bird}{\mathit{bird}}
\newcommand{\Tweety}{\mathit{tweety}}
\newcommand{\Skippy}{\mathit{skippy}}
\newcommand{\Rocky}{\mathit{rocky}}

% \newcommand{\Comp}{\mathsf{c}\,}
\newcommand{\trans}{\mathsf{trans}}

% \newcommand{\eqdef}{%
%   \mathrel{\vbox{\offinterlineskip\ialign{%
%     \hfil##\hfil\cr%
%     $\scriptscriptstyle\mathrm{def}$\cr%
%     \noalign{\kern1pt}%
%     $=$\cr%
%     \noalign{\kern-0.1pt}%
% }}}}


\newcommand{\WCS}{WCS\xspace}




\newcounter{bar}
\setcounter{bar}{-1}
\DeclareRobustCommand{\nr}[1]{%
   \refstepcounter{bar}%
   \thebar\label{#1}}


\newcounter{barp}
\setcounter{barp}{-1}
\DeclareRobustCommand{\nrp}[1]{%
   \refstepcounter{barp}%
   \thebarp\label{#1}}

\newcommand{\wcs}{\textsf{wcs}}
\newcommand{\asp}{\textsf{asp}}
\newcommand{\wcsp}{\textsf{wcs}-program\xspace}
\newcommand{\aspp}{\textsf{asp}-program\xspace}

\newcommand{\negClause}{\textsf{mod$_{\neg}$}}

\newcommand{\Nformulas}{\mbox{\textbf{N}-formulas}\xspace}
\newcommand{\Lformulas}{\mbox{\textbf{\L}-formulas}\xspace}
\newcommand{\Lpformulas}{\ensuremath{\textbf{\L}^{+}}\!-formulas\xspace}
\newcommand{\Nformula}{\mbox{\textbf{N}-formula}\xspace}
\newcommand{\Lformula}{\mbox{\textbf{\L}-formula}\xspace}
\newcommand{\Lpformula}{\ensuremath{\textbf{\L}^{\text{\tiny\!+}}}\!-formula\xspace}
\newcommand{\Itransformation}{\textbf{N}-transformation\xspace}
\newcommand{\Ltransformation}{\textbf{{\L}}-transformation\xspace}
\newcommand{\Ntheory}{\mbox{\textbf{N}-theory}\xspace}
\newcommand{\Ntheories}{\mbox{\textbf{N}-theories}\xspace}
\newcommand{\Lptheory}{\mbox{\ensuremath{\textbf{\L}^{\text{\tiny\!+}}}\!-theory}\xspace}
\newcommand{\Lptheories}{\mbox{\ensuremath{\textbf{\L}^{\text{\tiny\!+}}}\!-theories}\xspace}
\newcommand{\Ltheory}{\mbox{\textbf{\L}-theory}\xspace}
\newcommand{\Ltheories}{\mbox{\textbf{\L}-theories}\xspace}
\newcommand{\GammaL}{\Gamma^{\textbf{\tiny\L}}}
\newcommand{\GammaI}[1]{{\tilde{\textbf{N}}(#1)}}
% \newcommand{\GammaI}[1]{{\tilde{#1}}}

\newcommand{\NP}{{\textbf{N}(\CalP)}}
\newcommand{\NwoP}{{\textbf{N}}}
\newcommand{\NPI}{{\textbf{N}(\CalP^I)}}
\newcommand{\varphiI}{\textbf{N}(\varphi)}
\newcommand{\Lplogic}{\mbox{\textbf{\L\ensuremath{^{\text{\tiny\!+}}}}-logic}\xspace}
\newcommand{\Llogic}{\mbox{\textbf{\L}-logic}\xspace}
\newcommand{\Nlogic}{\mbox{\textbf{N}-logic}\xspace}
\newcommand{\HTlogic}{\textbf{HT}-logic\xspace}
\newcommand{\negnafClause}{\textsf{mod$_{\neg, \naf}$}}


\newcommand{\modelsLogic}{\models_{\text{\tiny \ensuremath{\CalL}}}}
\newcommand{\equivLogic}{\equiv_{\text{\tiny \ensuremath{\CalL}}}}

\newcommand{\impliesN}{\leftarrow_{\text{\rm\tiny C}}}
\newcommand{\dimpliesN}{\leftrightarrow_{\text{\tiny C}}}
\newcommand{\equivN}{\equiv_{\text{\tiny C}}}
\newcommand{\modelsN}{\models_{\text{\tiny C}}}


\newcommand{\impliesL}{\leftarrow_{\text{\rm \tiny \L}}}
\newcommand{\modelsL}{\models_{\text{\tiny \text{\rm \L}}}}
\newcommand{\equivL}{\equiv_{\text{\tiny \text{\rm \L}}}}
\newcommand{\dimpliesL}{\leftrightarrow_{\text{\rm \tiny \L}}}

\newcommand{\cMt}{\CalM^{t}}


\newcommand{\leftrightL}{\leftrightarrow_{\text{\tiny \L}}}
\newcommand{\leftrightI}{\leftrightarrow_{\text{\tiny N}}}

\newcommand{\impliesX}{\leftarrow_{\text{\rm\tiny X}}}

\newcommand{\equivX}{\equiv_{\text{\tiny X}}}
\newcommand{\modelsl}{\models_{\text{\tiny \L}}}
\newcommand{\equivl}{\equiv_{\text{\tiny \L}}}


\newcommand{\modelsHT}{\models_{\text{\tiny HT}}}
\newcommand{\modelsHTp}{\models^+_{\text{\tiny HT}}}
\newcommand{\modelsHTn}{\models^-_{\text{\tiny HT}}}


\def\modelsp{\models^+}
\def\modelsn{\models^-}



\newcommand{\dimpliesX}{\leftrightarrow_{\text{\tiny X}}}


% \def\at{\atoms(\CalP)}
\def\sI{\mathcal{I}}
\def\sJ{\mathcal{J}}
\def\sM{\mathcal{M}}
\newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand\htinterpretation{\mbox{HT-interpretation}\xspace}
\newcommand\htinterpretations{\mbox{HT-interpretations}\xspace}
\def\modelspm{\models^\pm}
% \newcommand{\set}[1]{\ensuremath{\{#1\}}}
% \newcommand{\setm}[2]{\ensuremath{\{\ #1\ \big|\ #2\ \}}}

\newcommand{\tranN}[1]{\ensuremath{\mathbf{N}(#1)}}
\newcommand{\tranL}[1]{\mbox{\ensuremath{\normalfont{\textbf{\L}}}}(#1)}

\newcommand{\reg}[1]{\ensuremath{\text{reg}(#1)}}
\newcommand{\ASP}[1]{\ensuremath{\text{ASP}(#1)}}
\newcommand{\Comp}[1]{\ensuremath{\textrm{\small c}(#1)}}
\newcommand{\wComp}[1]{\ensuremath{\textrm{\small wc}(#1)}}
% \newcommand{\nComp}[1]{\ensuremath{\textrm{\small dc}(#1)}}
\newcommand{\nComp}[1]{{\tilde{#1}}}


\newcommand{\dnComp}[1]{\ensuremath{\textrm{\small ddc}(#1)}}
\newcommand{\ctxtfree}[1]{\ensuremath{\text{ctxt-free}(#1)}}
\newcommand{\Pdisj}[1]{\ensuremath{\textrm{\small srf}(#1)}}
\newcommand{\supr}[1]{\ensuremath{\textrm{\small supr}(#1)}}
\newcommand{\WComp}[1]{\wComp{#1}}
\newcommand{\sing}[1]{\ensuremath{\tilde{\textrm{\small {no}}}(#1)}}
\def\wcmodel{\mbox{wc-model}\xspace}
\def\wcmodels{\mbox{wc-models}\xspace}
\def\wcsmpl{\mbox{wc-simple}\xspace}


\newcommand{\essay}{\mathit{e}}
\newcommand{\nessay}{\mathit{\overline{essay}}}
\newcommand{\library}{\mathit{library}}
% \newcommand{\nlibrary}{\mathit{\overline{library}}}
\newcommand{\lib}{\ell}
\newcommand{\nlib}{\overline{\ell}}
\newcommand{\ess}{e}
\newcommand{\add}{\open \rightarrow \lib}

% \newcommand{\tbook}{t}
% \newcommand{\ntbook}{\overline{t}}
\newcommand{\open}{o}
% \newcommand{\nopen}{\overline{o}}
\newcommand{\smpl}{e \leadsto \lib}
\newcommand{\rmpl}{t \leadsto \lib}

\def\sI{\mathcal{I}}
\def\sM{\mathcal{M}}
% \newcommand{\tuple}[1]{\ensuremath{\langle #1 \rangle}}
% \newcommand\htinterpretation{\mbox{HT-interpretation}\xspace}
% \newcommand\htinterpretations{\mbox{HT-interpretations}\xspace}
\def\modelsht{\models_{\mbox{\tiny \it{HT}}}}
\def\modelsp{\modelsht^+}
\def\modelsn{\modelsht^-}
\def\modelspm{\models^\pm}
% \newcommand{\set}[1]{\ensuremath{\{#1\}}}
% \newcommand{\setm}[2]{\ensuremath{\{\ #1\ \big|\ #2\ \}}}
